Nonlinear Functional Output Regression: a Dictionary Approach

To address functional-output regression, we introduce projection learning (PL), a novel dictionary-based approach that learns to predict a function that is expanded on a dictionary while minimizing an empirical risk based on a functional loss. PL makes it possible to use non orthogonal dictionaries and can then be combined with dictionary learning; it is thus much more flexible than expansion-based approaches relying on vectorial losses. This general method is instantiated with reproducing kernel Hilbert spaces of vector-valued functions as kernel-based projection learning (KPL). For the functional square loss, two closed-form estimators are proposed, one for fully observed output functions and the other for partially observed ones. Both are backed theoretically by an excess risk analysis. Then, in the more general setting of integral losses based on differentiable ground losses, KPL is implemented using first-order optimization for both fully and partially observed output functions. Eventually, several robustness aspects of the proposed algorithms are highlighted on a toy dataset; and a study on two real datasets shows that they are competitive compared to other nonlinear approaches. Notably, using the square loss and a learnt dictionary, KPL enjoys a particularily attractive trade-off between computational cost and performances.

==> main/related.tex <==
In this section, we present briefly four existing approaches to nonlinear FOR to which we compare our method in Section \ref{sec :: experiments}. \citet{BarathAl17} and \citet{PoczosAl15} are specific to functional data. While we propose a straightforward extension of the latter for non-functional input data, such extension is not possible for the former. 

\dimitri{Reléguer une partie en supplementary ?} \\
\noindent{\bf Functional kernel ridge regression (FKRR). }\citet{KadriAl10, KadriAl16} solves a functional KRR problem in the framework of function-valued-RKHSs (fv-RKHSs). To that end, they minimize the empirical risk $\frac 1 \nsamp \sum_{\sampiter=1}^\nsamp \| y_\sampiter - \regfunc(x_\sampiter) \|^2_{\cali Y} + \lambda \|\regfunc\|^2_{\cali H_{\Kxkadri}}$ over $\cali H_{\Kxkadri}$ the fv-RKHS associated to some OVK $\Kxkadri: \inspace \times \inspace \longrightarrow L(\cali Y)$, with $\cali Y$ a Hilbert space. That is very different from KPL. Indeed, in Problem \eqref{prob :: empirical risk dict vvrkhs}, we learn a vector-valued function which yields decomposition coefficients in a dictionary $\dict$, whereas \citet{KadriAl16} learns a function-valued function as follows. A representer theorem applies yielding the closed-form solution $( \Kxmatkadri + \lambda \matrb I)^{-1}\outsamp$ with $(\Kxmatkadri + \lambda \matrb I)^{-1} \in \boundedops(\cali Y)^{\nsamp \times \nsamp}$ and $\outsamp \in \cali Y^\nsamp$. Focusing on separable kernels $\Kxkadri(x_0, x_1)=k^{\text{in}}(x_0, x_1) \matop L$ with $k^{\text{in}}$ a scalar-valued kernel on $\inspace$ and $\matop L \in \boundedops(\cali Y)$ an integral operator associated to a scalar-valued kernel $k^{\text{out}}$ on $\outfuncdom^2$ and a measure $\mu$ on $\outfuncdom$; then $( \Kxmatkadri + \lambda \matrb I)^{-1}\outsamp = (\Kxinmatkadri \otimes \matop L + \lambda \matrb I)^{-1} \outsamp $. Two approaches are possible. \textbf{(i)} An eigendecomposition can be performed. If such decomposition of $\matop L$ is known in closed-form, the Kronecker product can be exploited to solve the system in $\cali O(\nsamp^3 + \nsamp^2 J t)$ time, with $J$ the number of eigenfunctions considered and $t$ the size of the discrete grid used to approximate functions in $\cali Y$. Unfortunately, such closed-forms are rarely known \citep[Section~4.3]{RasmussenWilliams06}. Notably one exists if $k^{\text{out}}(\theta_0, \theta_1) = \exp(-|\theta_0 - \theta_1 |)$, $\outfuncdom=[0, 1]$ and $\mu$ is the Lebesgue measure \citep{Hawkins89}, or if $k^{\text{out}}$ is a Gaussian kernel, $\outfuncdom = \bb R^q$ and $\mu$ is a Gaussian measure \citep{ZhuAl97}. Otherwise, an approximate eigendecomposition can be performed which adds a $\cali O(t^3)$ term to the above time complexity. \textbf{(ii)} The problem can be discretized on a regular grid \citep{KadriAl10}---time complexity $\cali O(\nsamp^3 + t^3 + \nsamp^2 t + \nsamp t)$ using a Sylvester solver.  To compare the above time complexities to that of KPL, we highlight that typically $t \gg \ndict$ and $t$ is at least of the same order as $\nsamp$. 

\noindent{\bf Triple basis estimator (3BE).}  \citet{PoczosAl15} firstly represent separately the input and output functions on truncated orthonormal bases obtaining decomposition coefficients $(\beta_\sampiter, \gamma_\sampiter)_{\sampiter=1}^\nsamp$, with for all $\sampiter \in [\nsamp]$, $\beta_\sampiter \in \bb R^c$ and $\gamma_\sampiter \in \bb R^\ndict$; $c \in \bb N^*$ being the cardinality of the input basis and $\ndict \in \bb N^*$ that of the output basis. The output coefficients  are then regressed on the input ones using approximate KRRs with RFFs \cite{RahimiRecht08} defined on the inputs. Using the ridge closed-form and putting aside the computations of the decomposition coefficients, solving 3BE has time complexity $\cali O(J^3 + J^2 \ndict)$ with $J$ the number of RFFs used. 3BE as proposed by \citet{PoczosAl15} is specific to function to function regression. As a consequence, when input data are not functional---as in Section \ref{subsec :: speech}---, we propose to directly deal with the input data through a kernel and call this extension \textbf{one basis estimator (1BE)}. We highlight that 1BE is then a particular case of KPL when the $\geneloss_2$ loss is used, $\dict$ is orthonormal and $\Kx = k \matop I$. In that case, the time complexity is $\cali O(\nsamp^3 + \nsamp^2 \ndict)$ since we need to solve $\ndict$ KRRs problems which share the same kernel matrix.  

\noindent{\bf Kernel additive model (KAM).} \citet{BarathAl17} builds on the additive function to function regression model using RKHSs. Taking $[0, 1]$ as input and output domain, they minimize: \\ $\sum_{\sampiter=1}^\nsamp \int_0^1 \left (y_\sampiter(\theta) - \int_0^1 \regfunc(\theta, \gamma, x_\sampiter(\gamma))d\gamma \right )^2 d \theta + \lambda \|\regfunc \|^2_{\cali H_{\Kxbarath}}$ over $\cali H_{\Kxbarath}$ the RKHS of a scalar-valued kernel $\Kxbarath: ([0, 1] \times [0, 1] \times \bb R)^2 \longrightarrow \bb R$ and $\lambda > 0$. A representer theorem leads to a closed-from solution. To alleviate the computations, a truncated basis of $J < \nsamp $ of empirical functional principal components of $(y_\sampiter)_{\sampiter=1}^\nsamp$ is used. A matrix of size $\nsamp J \times \nsamp J$ must then be inverted yielding a time complexity of $\cali O(\nsamp^3 J^3)$. 

\noindent{\bf Kernel Estimator (KE).} Finally, the functional Nadaraya-Watson kernel estimator has been studied in \citet{Ferraty2011} in the general setting of Banach spaces. Considering a kernel function $K: \bb R \longmapsto \bb R$ combined with a given semi-metric $S$ on $\inspace$, for all $x \in \inspace$, they use the following estimator: $\nicefrac{\sum_{\sampiter=1}^\nsamp K \circ S(x, x_\sampiter) y_\sampiter} {\sum_{\sampiter=1}^\nsamp K \circ S(x, x_\sampiter)}$.
